Fault-Tolerant Bounded Flow Preservers

Given a directed graph $G = (V, E)$ with $n$ vertices, $m$ edges and a designated source vertex $s\in V$, we consider the question of finding a sparse subgraph $H$ of $G$ that preserves the flow from $s$ up to a given threshold $\lambda$ even after failure of $k$ edges. We refer to such subgraphs as $(\lambda,k)$-fault-tolerant bounded-flow-preserver ($(\lambda,k)$-FT-BFP). Formally, for any $F \subseteq E$ of at most $k$ edges and any $v\in V$, the $(s, v)$-max-flow in $H \setminus F$ is equal to $(s, v)$-max-flow in $G \setminus F$, if the latter is bounded by $\lambda$, and at least $\lambda$ otherwise. Our contributions are summarized as follows: 1. We provide a polynomial time algorithm that given any graph $G$ constructs a $(\lambda,k)$-FT-BFP of $G$ with at most $\lambda 2^kn$ edges. 2. We also prove a matching lower bound of $\Omega(\lambda 2^kn)$ on the size of $(\lambda,k)$-FT-BFP. In particular, we show that for every $\lambda,k,n\geq 1$, there exists an $n$-vertex directed graph whose optimal $(\lambda,k)$-FT-BFP contains $\Omega(\min\{2^k\lambda n,n^2\})$ edges. 3. Furthermore, we show that the problem of computing approximate $(\lambda,k)$-FT-BFP is NP-hard for any approximation ratio that is better than $O(\log(\lambda^{-1} n))$.

==> opt.tex <==
\section{Computing Optimal $k$-FT-BFP and $k-$FTRS}

\Keerti{Question: Can we compute an optimal $k$-FTRS in $n^{O(k)}$ time?
Similarly, can we compute optimal $(\lambda,1)$-\ftbfp~ in $n^{O(\lambda+k)}$ time}


\subsection{Verifying Optimal FTRS}


\begin{lemma}

Let $s$ be a source, $t$ be a destination, and $E_t$ be set of in-edges to $t$ and $G_t$ be graph obtained from $G$
when in-edges of $t$ is restricted to $E_t$.

Let $(A,B)$ be partition of $V$ induced by $\fmc(s,t,G)$, and $C$ be set of in $E\cap (A\times B)$.



Then, $E_t$ is sufficient set of in-edges for $k$-$\ftrs(t)$
if and only if for all $F\subset C$,

$G_t\setminus F$ is 
a $ k - |F|$ - \ftrs~ for the graph  $G \setminus F$ with respect to $A\cup \Out(A)$ as source.
\end{lemma}

\Harsh{(Condition that $k\geq|C|$) and $(A\cup \Out(C \setminus F)) \setminus {t}$ as Source}

Consider a fault $P$ for which $\exists$ a $s-t$ path in $G$ but not in $G_t$. \\ 
Let $B_r$ be $\subset out(A)$ reachable from $s$ in $G\setminus(P\cup E_t(v))$ and $B_r'$ be $\subset out(A)$ reachable from $s$ in $G_t\setminus(P\cup E_t(v))$. Since we sparsify $E_t(v)$ in $G$ and $G_t$ thus $B_r$ will be same as $B_r'$. \\

\begin{lemma} $\sum_{\forall i \in Out(A) \setminus B_r}|C \cap E_t(i)|$ $\leq$ $(A \times V) \cap P$. 
\end{lemma}

Consider $s-t$ max-flow in $G$. Since $C$ is a min-cut by min-cut max-flow theorem there exist $|C|$ disjoint paths from $s-t$ paths in $G$ let $S_p$ be the set of all these paths. 
Each path $p$ in $S_p$ will have exactly 1 and unique edge $e_p$ in it from C. Using this property we define a set $T_i$ for all vertices i in Out(A) 

$$T_i = \{ p : p \in S_p \ and \ out(e_p) = i \} $$

For each vertex $i$ in $Out(A)$,$T_i$ will have $ |C \cap E_t(i)| $ paths in it and each path will belong to only one such set $T$. Now for a
destination set $Out(A) \setminus B_r$ consider the set of disjoint paths $$S_{paths} = \bigcup\limits_{i \in Out(A) \setminus B_r} T_{i}$$

Now for each path $p$ in $S_{paths}$ replace $p$ with subpath $p[s,out(e_p)]$ in $S_{paths}$ which lies entirely in $A \times V$. Now since
 $\Out(A) \setminus B_r$ is not reachable from $s$ all these paths either have an edge from $P$ or $E_t$. For all $p \in S_{paths}$ such that 
$p$ is not an $s-t$ atleast an edge from it will be a part of $P$ as $t$ is not present in these paths hence no edge from $E_t(v)$ \\ 
Now for all the paths $p \in S_{paths}$ which end at $t$ they too will have an edge from it in $P$. This can be proved via contradiction as consider one such path $p$ which has no such fault. Now considering $F$ to be $C \setminus e_p$.
$G_t$ should be $ k - |C| + 1$ - \ftrs~ for the graph $G \setminus F$ with respect to $(A\cup \Out(A))\setminus t$ 
which ensures that $e_p$ will be included in $G_t$ thus $p$ will be completely intact in $G_t \setminus P$ which contradicts our initial 
assumption of $P$. Hence all such paths will to have an edge in $P$. 
Thus for each path in $S_{paths}$ one of their edge is present in $P$ hence $(A \times V) \cap P$  is atleast $|S_{paths}|$ which is $\sum_{\forall i \in Out(A) \setminus B_r}|C \cap E_t(i)|$ as all paths are disjoint.  \\ 

Consider the set $K$ such that  
$$K = \{ e : e \in C \ \& \ out(e) \in (\Out(A) \setminus B_r) \}$$ 

\begin{lemma}
$\exists$ a $s-t$ path in $G \setminus (K \cup P)$ if $\exists$ a $s-t$ path in $G \setminus P$. \\
\end{lemma}
If the $s-t$ path in $G \setminus P$ doesn't contain an edge from $K$  the same path will also exist in $G \setminus (K \cup P)$ thus the 
lemma holds for this case. Now let the $s-t$ in  $G \setminus P$  contains an edge $e$ from $K$ now by definition of $B_r$ $out(e)$ was not 
reachable from $s$ in $G\setminus(P \cup E_t)$ Hence this path also contains an edge $e'$ from $E_t$ Hence subpath $s-out(e')$ is also an 
$s-t$ path without $e$.Thus we can always remove any edges in $K$ from such an $s-t$ path to get an $s-t$ path without any edges of $K$ 
hence if $\exists$ a $s-t$ path in $G \setminus (K \cup P)$ if $\exists$ a $s-t$ path in $G \setminus P$. \\ 

%%. By above lemmas if there exist a $s-t$ path in $G \setminus (K \cup P)$ if $\exists$ a $s-t$ path in $G \setminus P$.Now if there is no $s-t$ path in $G_t \setminus P$ but there is one in $G \setminus P$ there must exist a fault $L$ 
Now consider the graph $G_t \setminus K$ which is a $ k - |K|$ - FTRS for the source $A \cup B_r$. By above lemmas we know there exist a $s-t$ path in 
$G \setminus (K \cup P)$ if $\exists$ a $s-t$ path in $G \setminus P$. Thus if there is an $s-t$ path in $G \setminus P$ there is an  $(A \cup B_r) - t$ 
path in $G \setminus K$. Thus if there is no such $s-t$ path in $G_t \setminus K$, $P \cap (B\times B) \geq  k - |K| + 1 $. 
From lemma 4.2 we know $|K| \leq$ $(A \times V) \cap P$ now since $(A \times V)$ and $B \times B$ are disjoint $P$ is atleast of size $k + 1$ thus our graph 
is an $k$-$\ftrs(t)$.

\paragraph{Proof of necessity}

Consider a set $F \subset C$ for which  $G_t$ is not $ k - |F|$ - FTRS over the graph $G \setminus F$.
Now since $G_t \setminus F$ which is not a $ k - |F|$ - FTRS $\exists$ a fault $P'$ for which there is an $A \cup Out(C \setminus F) - t$ path in $G$
but not in $G_t$ where $|P'| \leq k - |F|$. Now consider a fault $$P = F \ \cup  P'$$ Size of $P$ will be $|P| \leq |F| + |P'| $ hence $|P| \leq k$ and 
by construction there is and $s-t$ path in $G \setminus P$ but not in $G_t \setminus P$ hence $G_t$ is not a $\kftrs$ and the above given condition is 
necessary too.

\paragraph{Algorithm to verifying correctness}

\vspace{5cm}
\begin{algorithm}[!ht]
\BlankLine
\DontPrintSemicolon
\SetKwFunction{FCheckFTRS}{CheckFTRS}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FCheckFTRS{$S$,$G$,$G_t$,$t$,$k$}}{
    $C \gets \fmc(S,t,G)$ and $(A,B)$ be partition of $V(G)$ induced by $C$\;
    \uIf{$|C| > k$}{
        \KwRet\ ($|\fmc(S,t,G_t)| > k $)\;
    }
    \ForEach{$J\subseteq C$}{
        $P \gets \Out(C/J)$\;
        \uIf{$! CheckFTRS(S \cup A \cup P,G,G_t,t,k-|J|)$}{
            \KwRet\ false\;
        }
    }
    \KwRet\ true;
}
\;
\caption{Algorithm for verifying $\kftrs(t)$}
\label{algo:kFTRS(t)}
\end{algorithm}


\paragraph{Analysis of time complexity}

$$ T(k,r) = \sum_{i=0}^{r-1} T(k-i,r-i+1) \times  {}^{r}C_{i} + m(r+1) $$

and the simpler version  

$$ T(k) = \sum_{i=1}^{r-1} T(i) \times {}^{k+1}C_{i+1} + (k+1)m$$

which leads to the solution $A052882 \times m$ 
\newpage


\paragraph{Remark/ Paragraph on Computing optimal $k$-FTRS}




